HateXScore: A Metric Suite for Evaluating Reasoning Quality in Hate Speech Explanations

Hateful speech detection is a key component of content moderation, yet current evaluation frameworks rarely assess why a text is deemed hateful. We introduce \textsf{HateXScore}, a four-component metric suite designed to evaluate the reasoning quality of model explanations. It assesses (i) conclusion explicitness, (ii) faithfulness and causal grounding of quoted spans, (iii) protected group identification (policy-configurable), and (iv) logical consistency among these elements. Evaluated on six diverse hate speech datasets, \textsf{HateXScore} is intended as a diagnostic complement to reveal interpretability failures and annotation inconsistencies that are invisible to standard metrics like Accuracy or F1. Moreover, human evaluation shows strong agreement with \textsf{HateXScore}, validating it as a practical tool for trustworthy and transparent moderation. \textcolor{red}{Disclaimer: This paper contains sensitive content that may be disturbing to some readers.}

==> checklist.tex <==
\makeatletter
\@ifundefined{isChecklistMainFile}{
  % We are compiling a standalone document
  \newif\ifreproStandalone
  \reproStandalonetrue
}{
  % We are being \input into the main paper
  \newif\ifreproStandalone
  \reproStandalonefalse
}
\makeatother

\ifreproStandalone
% \documentclass[letterpaper]{article}
% \usepackage[submission]{aaai2026}
\setlength{\pdfpagewidth}{8.5in}
\setlength{\pdfpageheight}{11in}
% \usepackage{times}
% \usepackage{helvet}
% \usepackage{courier}
% \usepackage{xcolor}
\frenchspacing

% \begin{document}
% \fi
\setlength{\leftmargini}{20pt}
\makeatletter\def\@listi{\leftmargin\leftmargini \topsep .5em \parsep .5em \itemsep .5em}
\def\@listii{\leftmargin\leftmarginii \labelwidth\leftmarginii \advance\labelwidth-\labelsep \topsep .4em \parsep .4em \itemsep .4em}
\def\@listiii{\leftmargin\leftmarginiii \labelwidth\leftmarginiii \advance\labelwidth-\labelsep \topsep .4em \parsep .4em \itemsep .4em}\makeatother

\setcounter{secnumdepth}{0}
\renewcommand\thesubsection{\arabic{subsection}}
\renewcommand\labelenumi{\thesubsection.\arabic{enumi}}

\newcounter{checksubsection}
\newcounter{checkitem}[checksubsection]

\newcommand{\checksubsection}[1]{%
  \refstepcounter{checksubsection}%
  \paragraph{\arabic{checksubsection}. #1}%
  \setcounter{checkitem}{0}%
}

\newcommand{\checkitem}{%
  \refstepcounter{checkitem}%
  \item[\arabic{checksubsection}.\arabic{checkitem}.]%
}
\newcommand{\question}[2]{\normalcolor\checkitem #1 #2 \color{blue}}
\newcommand{\ifyespoints}[1]{\makebox[0pt][l]{\hspace{-15pt}\normalcolor #1}}

\section*{Reproducibility Checklist}

\vspace{1em}
\hrule
\vspace{1em}

\textbf{Instructions for Authors:}

This document outlines key aspects for assessing reproducibility. Please provide your input by editing this \texttt{.tex} file directly.

For each question (that applies), replace the ``Type your response here'' text with your answer.

\vspace{1em}
\noindent
\textbf{Example:} If a question appears as
%
\begin{center}
\noindent
\begin{minipage}{.9\linewidth}
\ttfamily\raggedright
\string\question \{Proofs of all novel claims are included\} \{(yes/partial/no)\} \\
Type your response here
\end{minipage}
\end{center}
you would change it to:
\begin{center}
\noindent
\begin{minipage}{.9\linewidth}
\ttfamily\raggedright
\string\question \{Proofs of all novel claims are included\} \{(yes/partial/no)\} \\
yes
\end{minipage}
\end{center}
%
Please make sure to:
\begin{itemize}\setlength{\itemsep}{.1em}
\item Replace ONLY the ``Type your response here'' text and nothing else.
\item Use one of the options listed for that question (e.g., \textbf{yes}, \textbf{no}, \textbf{partial}, or \textbf{NA}).
\item \textbf{Not} modify any other part of the \texttt{\string\question} command or any other lines in this document.\\
\end{itemize}

You can \texttt{\string\input} this .tex file right before \texttt{\string\end\{document\}} of your main file or compile it as a stand-alone document. Check the instructions on your conference's website to see if you will be asked to provide this checklist with your paper or separately.

\vspace{1em}
\hrule
\vspace{1em}

% The questions start here

\checksubsection{General Paper Structure}
\begin{itemize}

\question{Includes a conceptual outline and/or pseudocode description of AI methods introduced}{(yes/partial/no/NA)}
yes

\question{Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results}{(yes/no)}
yes

\question{Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper}{(yes/no)}
yes

\end{itemize}
\checksubsection{Theoretical Contributions}
\begin{itemize}

\question{Does this paper make theoretical contributions?}{(yes/no)}
no

	\ifyespoints{\vspace{1.2em}If yes, please address the following points:}
        \begin{itemize}
	
	\question{All assumptions and restrictions are stated clearly and formally}{(yes/partial/no)}
	NA

	\question{All novel claims are stated formally (e.g., in theorem statements)}{(yes/partial/no)}
        NA

	\question{Proofs of all novel claims are included}{(yes/partial/no)}
	NA

	\question{Proof sketches or intuitions are given for complex and/or novel results}{(yes/partial/no)}
	NA

	\question{Appropriate citations to theoretical tools used are given}{(yes/partial/no)}
	NA

	\question{All theoretical claims are demonstrated empirically to hold}{(yes/partial/no/NA)}
	NA

	\question{All experimental code used to eliminate or disprove claims is included}{(yes/no/NA)}
	NA
	
	\end{itemize}
\end{itemize}

\checksubsection{Dataset Usage}
\begin{itemize}

\question{Does this paper rely on one or more datasets?}{(yes/no)}
yes

\ifyespoints{If yes, please address the following points:}
\begin{itemize}

	\question{A motivation is given for why the experiments are conducted on the selected datasets}{(yes/partial/no/NA)}
	yes

	\question{All novel datasets introduced in this paper are included in a data appendix}{(yes/partial/no/NA)}
	NA

	\question{All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes}{(yes/partial/no/NA)}
	NA

	\question{All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations}{(yes/no/NA)}
	yes

	\question{All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available}{(yes/partial/no/NA)}
	yes

	\question{All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing}{(yes/partial/no/NA)}
	NA

\end{itemize}
\end{itemize}

\checksubsection{Computational Experiments}
\begin{itemize}

\question{Does this paper include computational experiments?}{(yes/no)}
yes

\ifyespoints{If yes, please address the following points:}
\begin{itemize}

	\question{This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting}{(yes/partial/no/NA)}
	yes

	\question{Any code required for pre-processing data is included in the appendix}{(yes/partial/no)}
	partial

	\question{All source code required for conducting and analyzing the experiments is included in a code appendix}{(yes/partial/no)}
	partial

	\question{All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes}{(yes/partial/no)}
	yes
        
	\question{All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from}{(yes/partial/no)}
	yes

	\question{If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results}{(yes/partial/no/NA)}
	yes

	\question{This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks}{(yes/partial/no)}
	yes

	\question{This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics}{(yes/partial/no)}
	yes

	\question{This paper states the number of algorithm runs used to compute each reported result}{(yes/no)}
	yes

	\question{Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information}{(yes/no)}
	yes

	\question{The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank)}{(yes/partial/no)}
	yes

	\question{This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments}{(yes/partial/no/NA)}
	yes


\end{itemize}
\end{itemize}
\ifreproStandalone
% \end{document}
% \fi

==> model.tex <==

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.95\textwidth]{images/pipeline.png}
  \caption{Self-training pipeline for offensive content detection using Multi-Agent Vision-Language Models (MA-VLMs).}
  \label{fig:pipeline}
\end{figure*}

Assume an offensive content detection dataset of $N$ samples, with only $n \ll N$ labeled. The objective is to effectively leverage both the limited labeled data and the unlabeled data to improve model performance. Figure~\ref{fig:pipeline} presents the overall pipeline of our proposed approach, which employs an iterative self-training strategy. A lightweight classifier is used for training, while both the classifier and a Multi-Agent Vision-Language-Models (MA-VLMs) are utilized for pseudo-label generation.




\subsection{Self-Training Procedure}

The classifier model is trained via an iterative five-step self-training procedure:

\begin{enumerate}
    \item \textbf{Initial Training:} The classifier is first trained using only the \( n \) labeled samples.
    
    \item \textbf{Classifier Predict and Order:} The trained classifier is used to predict labels for the unlabeled set. All predictions are ranked based on the classifier's confidence scores.
    
    \item \textbf{MA-VLMs Agree or Disagree:} The top-\( k \) most confident predictions are selected and evaluated by a Multi-Agent Vision-Language Model (MA-VLM). If the MA-VLM agrees with the classifier’s prediction, the sample is pseudo-labeled as Agreed-Hateful/Offensive/Misogyny/Negative-Unknown or Agreed-Normal/Positive-Unknown, depending on the task. Otherwise, it is labeled as \textit{Disagreed-Unknown}.
    
    \item \textbf{Dataset Update and Retraining:} Both Agreed and Disagreed samples are removed from the unlabeled pool and added to the training set. The classifier is then retrained on the updated dataset using a novel PNU loss $L_{PNU}$, which incorporates contributions from Known, Agreed-Unknown, and Disagreed-Unknown samples.    
    \item \textbf{Validation Check:} If classifier performance on a development set improves, the process continues to the next iteration. Otherwise, the classifier is reverted to the previous round, and the current round's pseudo-labeled samples are discarded.
\end{enumerate}

The procedure terminates when all unlabeled samples have been either incorporated into the training set or discarded.


\subsection{Multi-Agent Vision-Language-Models (MA-VLMs)}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{images/MA_VLMs.png}
  \caption{Inference procedure of Multi-Agent Vision-Language Models (MA-VLMs) for offensive content detection, exemplified by a hate speech task: An unknown input is pseudo-labeled as Agreed-Hateful-Unknown or Agreed-Normal-Unknown if the Classifier model, Auditor VLM, and User VLM all concur. Otherwise, it is labeled as Disagreed-Unknown.}
  \label{fig:MA_VLMs}
\end{figure}

To emulate real-world auditing of online offensive content—where an auditor flags content, a user responds, and a final decision is made through dialogue—we propose a Multi-Agent Vision-Language-Models (MA-VLMs) framework, illustrated in Figure~\ref{fig:MA_VLMs}. It involves two distinct VLMs with contrasting personas: a strict auditor focused on detecting hate speech and a lenient user prioritizing free expression. Each agent provides an initial label and rationale, reviews the other's perspective, and then issues a final decision. Agreement is reached only when both agents agree with the classifier’s prediction; otherwise, the input is marked as disagreed.

\subsection{Positive-Negative-Unknown (PNU) Loss}
To fully utilize both known and unknown data, we propose a unified \textbf{PNU Loss} that incorporates Known, Agreed-Unknown, and Disagreed-Unknown samples. The overall loss is formulated as:

\begin{equation}
\mathcal{L} = (1 - \theta) \cdot (\mathcal{L}_{\text{PN}} + \mathcal{L}_{\text{soft-PN}}) + \theta \cdot \mathcal{L}_{\text{PU}}
\end{equation}

where $\theta \in [0, 1]$ controls the influence of PU learning.

The \textbf{PN loss} is a standard binary classification loss applied to Known data, where Hateful/Offensive/Misogyny/Negative classes are treated as positive ($y=1$) and Normal/Positive are treated as negative ($y=0$):


\begin{equation}
\mathcal{L}_{\text{PN}} = \pi_p \cdot \hat{R}_p^+ + (1 - \pi_p) \cdot \hat{R}_n^-
\end{equation}
\[
\quad \left\{
\begin{array}{l}
\hat{R}_p^+ = \frac{1}{n^p} \sum_{i=1}^{n^{p}} l(g(x_i^p), 1) \\
\hat{R}_n^- = \frac{1}{n^n} \sum_{i=1}^{n^{p}}  l(g(x_i^n), 0)
\end{array}
\right.
\]


Here, $\pi_p$ is the prior probability of the positive class, $l$ is the cross-entropy loss, and $g(x)$ denotes the model prediction. $x_i^p$ and $x_i^n$ represent samples with labels positive and negative, respectively, while $n^p$ and $n^n$ denote their corresponding sample counts.

The \textbf{soft-PN loss} leverages Agreed-Unknown samples, assigning soft labels to reflect uncertainty:

\begin{equation}
\mathcal{L}_{\text{soft-PN}} = \pi_p \cdot \hat{R}_{up}^+ + (1 - \pi_p) \cdot \hat{R}_{un}^-
\end{equation}
\[
\quad \left\{
\begin{array}{l}
\hat{R}_{up}^+ = \frac{1}{n^{up}} \sum_{i=1}^{n^{up}} l(g(x_i^{up}), 0.67) \\
\hat{R}_{un}^- = \frac{1}{n^{un}} \sum_{i=1}^{n^{un}} l(g(x_i^{un}), 0.33)
\end{array}
\right.
\]


Finally, the \textbf{PU loss} handles Disagreed Unknown samples using positive-unlabeled (PU) learning to extract weak supervision:

\begin{equation}
\mathcal{L}_{\text{PU}} = \pi_p ( \hat{R}_p^+ +\hat{R}_{up}^+ ) + \max\left(0, \hat{R}_u^--\pi_p \cdot (\hat{R}_p^-+\hat{R}_{up}^- ) )
\end{equation}
\[
\quad \left\{
\begin{array}{l}
\hat{R}_{u}^- = \frac{1}{n^{u}} \sum_{i=1}^{n^{u}} l(g(x_i^u), 0) \\
\hat{R}_p^+ = \frac{1}{n^p} \sum_{i=1}^{n^{p}} l(g(x_i^p), 0) \\
\hat{R}_{up}^+ = \frac{1}{n^{up}} \sum_{i=1}^{n^{up}} l(g(x_i^{up}), 0.33) \\
\end{array}
\right.
\]


This formulation enables the model to benefit from both strong supervision (known data) and weak supervision (unknown data), without discarding valuable information.

